Modeling Multi-hop Question Answering as Single Sequence Prediction

Fusion-in-decoder (Fid) (Izacard and Grave, 2020) is a generative question answering (QA) model that leverages passage retrieval with a pre-trained transformer and pushed the state of the art on single-hop QA. However, the complexity of multi-hop QA hinders the effectiveness of the generative QA approach. In this work, we propose a simple generative approach (PathFid) that extends the task beyond just answer generation by explicitly modeling the reasoning process to resolve the answer for multi-hop questions. By linearizing the hierarchical reasoning path of supporting passages, their key sentences, and finally the factoid answer, we cast the problem as a single sequence prediction task. To facilitate complex reasoning with multiple clues, we further extend the unified flat representation of multiple input documents by encoding cross-passage interactions. Our extensive experiments demonstrate that PathFid leads to strong performance gains on two multi-hop QA datasets: HotpotQA and IIRC. Besides the performance gains, PathFid is more interpretable, which in turn yields answers that are more faithfully grounded to the supporting passages and facts compared to the baseline Fid model.

==> source/broader_impact.tex <==
%\paragraph{Broader Impact}
\vspace{-6pt}
\section*{Broader Impact}
\vspace{-6pt}
Our work advances the generative QA approach in the context of complex, multi-hop QA.
The generative QA approach has pushed state of the art of single-hop open-domain QA benchmarks, and multi-hop QA is a fundamental research area to develop complex reasoning abilities in QA models.
This paper contributes toward the goal of improving real-world QA systems to handle more complex questions in interpretable ways.
However, there is still much room for investigation, and more research efforts are encouraged to bridge the gap between the research and real use cases.

Incorporating an interpretability into the generative QA approach is an important step towards our goal, but it is still implicit through the self-attention mechanism trained with an end-to-end training objective.
We encourage the research community to explore more explicit grounding process, instead of completely relying on the transformer model architectures.
We also need in-depth investigation on the reasoning ability of the generative QA approach in open-domain QA scenarios.

Lastly, there is large room for investigation on what are the significant factors that affect the reasoning ability.
It is common to use large pre-trained (transformer) models, but it is not clear which factors affect the QA performance more, the pre-training objective, the model architecture, the model size, or the corpus used for the pre-training.
Understanding these aspects is important in capturing the fundamental research direction to be focused in future work.
